Algebraic and Analytic Approaches for Parameter Learning in Mixture Models

We present two different approaches for parameter learning in several mixture models in one dimension. Our first approach uses complex-analytic methods and applies to Gaussian mixtures with shared variance, binomial mixtures with shared success probability, and Poisson mixtures, among others. An example result is that $\exp(O(N^{1/3}))$ samples suffice to exactly learn a mixture of $k<N$ Poisson distributions, each with integral rate parameters bounded by $N$. Our second approach uses algebraic and combinatorial tools and applies to binomial mixtures with shared trial parameter $N$ and differing success parameters, as well as to mixtures of geometric distributions. Again, as an example, for binomial mixtures with $k$ components and success parameters discretized to resolution $\epsilon$, $O(k^2(N/\epsilon)^{8/\sqrt{\epsilon}})$ samples suffice to exactly recover the parameters. For some of these distributions, our results represent the first guarantees for parameter estimation.

==> 04-conclusion.tex <==
\section{Conclusion}

\andrew{akshay: can you think about this after the dust has settled elsewhere?}

conjecture that some of our results are tight?

==> extendedproof.tex <==


In this setting, let us assume that we have two mixtures of Gaussian distributions $\mathcal{M}$ and $\mathcal{M'}$ each containing $k$ components i.e. 
 $\mathcal{M} =
  \frac{1}{k}\sum_{i=1}^k \Nc(\mu_i,\sigma)$
and 
$\mathcal{M}' =
  \frac{1}{k}\sum_{i=1}^k \Nc(\mu_i',\sigma)$
where 
\[\mu_i, \mu_i' \in \{\ldots, -2\epsilon, -\epsilon, 0,\epsilon, 2\epsilon \ldots \} \]

Define $\mathcal{A}\equiv \{\mu_i\}_{i=1}^{i=k}$ to be the set of means corresponding to the components in mixture $\mathcal{M}$ and similarly define the analogous set $\mathcal{B}\equiv \{\mu_i'\}_{i=1}^{i=k}$ corresponding to the mixture $\mathcal{M}'$. Now it is well known that the moment generating function of a random variable $X \sim \mathcal{N}(\mu,\sigma^2)$ distributed according to a Gaussian distribution is given by 
\begin{align*}
C(X)=\avg (e^{t})^{X}=e^{t\mu+\frac{t^{2}\sigma^{2}}{2}}
\end{align*}   
From now on, we will take $t$ to be a complex number of the form $\alpha+i \beta$ and let $w$ be the complex number $e^{\alpha+i \beta}$. Therefore for the two random variables $X \sim \mathcal{M}$ and $X' \sim \mathcal{M}'$, we must have that 
\begin{align*}
C(X)-C(X') = \frac{1}{k}  e^{\frac{(\alpha+i \beta)^{2} \sigma^{2}}{2}} \Big(\sum_{a \in A} e^{a(\alpha+i \beta)}- \sum_{b \in B} e^{b(\alpha+i\beta)} \Big)
\end{align*}
Define $\mu_{\max}$ and $\mu_{\min}$ be the largest and smallest number in the set $A \cup B \setminus A \cap B$ respectively. In that case we must have 
\begin{align*}
|C(X)-C(X')|=\frac{1}{k}  e^{\frac{(\alpha^{2}-\beta^{2}) \sigma^{2}}{2}+\alpha\mu_{\min}} \lvert\Big(\sum_{a \in A} w^{a-\mu_{\min}}- \sum_{b \in B} w^{b-\mu_{\min}} \Big)\rvert
\end{align*}
%Now according to Corollary 3.2 of Borwein and Erdelyi, we have that for a complex polynomial $A(z)=\sum_j a_j z^j$ where $\max_j |a_j| \le M, |a_0|=1$ and a subarc of the unit circle in the complex plane $C$ with $\ell(C)=a$
%\begin{align*}
%\sup_{z \in C} A(z) \ge \exp (-\frac{c(1+\log M)}{a})
%\end{align*}
Since the mean parameters of the mixture lies on the grid $\{\dots,-2\epsilon,-\epsilon,0,\epsilon,2\epsilon,\dots\}$, define another complex number $w'$ such that $w=w'^{\frac{1}{\epsilon}}$. Now we have that
\begin{align*}
|C(X)-C(X')| = \frac{1}{k}  e^{\frac{(\alpha^{2}-\beta^{2}) \sigma^{2}}{2}+\alpha\mu_{\min}} \lvert \Big(\sum_{a \in A} w'^{\frac{a-\mu_{\min}}{\epsilon}}- \sum_{b \in B} w'^{\frac{b-\mu_{\min}}{\epsilon}} \Big) \rvert.
\end{align*}
Notice that $A(w')= \sum_{a \in A} w'^{\frac{a-\mu_{\min}}{\epsilon}}- \sum_{b \in B} w'^{\frac{b-\mu_{\min}}{\epsilon}} $ is a polynomial in $w'$ and therefore it is an entire function i.e. it is differentiable in the entire complex domain. Now consider a closed domain $Z=\{z \mid |z| \le r\}$ where $r=e^{\alpha \epsilon}$. Moreover define $\lambda=\sup_{arg(w') \in (-\frac{\pi}{L},\frac{\pi}{L})} |A(w')|$ and the polynomial $F(w')=\Pi_{j=0}^{L-1} A(w'e^{\frac{2\pi ij}{L}})$. Again, $F(w')$ is an entire function since it is a product of polynomials and therefore, by the maximum modulus principle, the function $F(w')$ attains its maximum on the boundary of the domain i.e. there exists $w^{\star} \in Z$ such that $|w^{\star}|=r$ for which 
\begin{align*}
|F(w^{\star})| \ge |F(0)| 
\end{align*}
Now, trivially we have that $|A(w')| \le 2kr^{\frac{\mu_{\max}-\mu_{\min}}{\epsilon}}$ and $|F(0)|=1$. Since we know that one of the factors of $F(w')$ is less than $\lambda$, we must have that $|F(w^{\star})| \le \lambda \Big(2kr^{\frac{\mu_{\max}-\mu_{\min}}{\epsilon}}\Big)^{L}$ and therefore,
\begin{align*}
\lambda \ge e^{-L \log 2r^{\frac{\mu_{\max}-\mu_{\min}}{\epsilon}}}=e^{-L(\log 2k+\alpha(\mu_{\max}-\mu_{\min}))}.
\end{align*}
Putting together all of the above, we have that 
\begin{align*}
|C(X)-C(X')| \ge \frac{1}{k}  e^{\frac{(\alpha^{2}-\beta^{2}) \sigma^{2}}{2}+\alpha\mu_{\min}-L(\log 2k+\alpha(\mu_{\max}-\mu_{\min}))}
\end{align*}
Let us denote $f_{\mathcal{M}},f_{\mathcal{M}'}$ as the probability measures corresponding to the mixtures $\mathcal{M},\mathcal{M'}$ respectively. Again, we can bound $|C(X)-C(X')|$ from above as shown below:
\begin{align*}
|C(X)-C(X')| &\le \bigintssss  |f_{\mathcal{M}}(x)w^{x}-f_{\mathcal{M'}}(x)w^{x}|dx \\
&\le \bigintssss_{x<t}  |f_{\mathcal{M}}(x)-f_{\mathcal{M'}}(x)||w|^{t}dx+\bigintssss_{x>t}|f_{\mathcal{M}}(x)|w^{x}dx+\bigintssss_{x>t}|f_{\mathcal{M'}}(x)|w^{x}dx  \\
& \le |w|^{t} \norm{\mathcal{M}-\mathcal{M'}}_{TV} +\frac{\avg |w|^{2X}}{|w|^{t-1}}+\frac{\avg |w|^{2X'}}{|w|^{t-1}}\\
&\le |w|^{t} \norm{\mathcal{M}-\mathcal{M'}}_{TV}+e^{(2\mu_{\max}\log |w|+2(\log |w|)^{2}\sigma^{2})-(t-1)\log |w|}
\end{align*}
It is evident that for $t=6 \mu_{\max}+6.5\sigma^{2}\alpha$ (Since $\alpha=\log |w|$) is sufficient to make the quantity $e^{(2\mu_{\max}\log |w|+2(\log |w|)^{2}\sigma^{2})-(t-1)\log |w|}$ exponentially small in both the mean and variance.
Also since the argument of the complex number $w'$ varies in the small arc around zero, we have that $\beta \in [-\frac{\pi}{\epsilon L},\frac{\pi}{\epsilon L}]]$. In that case we have that 
\begin{align}
\norm{\mathcal{M}-\mathcal{M'}}_{TV} \ge \frac{1}{k} \sup_{\alpha,L} \exp\Big(\alpha \mu_{\min}+\frac{\sigma^{2} \alpha^{2}}{2} -\frac{\sigma^{2} \pi^{2}}{2\epsilon^{2}L^{2}}-6\alpha\mu_{\max}-6.5\alpha^{2}\sigma^{2}-L(\log 2+\alpha(\mu_{\max}-\mu_{\min})) \Big)
\end{align}
Ignoring constants, we can substitute $L$ such that $\frac{\sigma^{2} \pi^{2}}{\epsilon^{2}L^2}=L(1+\alpha \Delta)$ and we have that 
\begin{align}
\norm{\mathcal{M}-\mathcal{M'}}_{TV} \ge \frac{1}{k} \sup_{\alpha} \exp\Big( \alpha \mu_{\min}-6\alpha\mu_{\max}-6\alpha^{2}\sigma^{2}-\Big(\frac{\sigma(1+\alpha (\mu_{\max}-\mu_{\min}))}{\epsilon}\Big)^{2/3} \Big)
\end{align}
For $\alpha=0$, we get back what we had before. Differentiating the expression within the $\exp(.)$ (which is concave and therefore has a supremum) and equating it to zero, we have that
\begin{align*}
\mu_{\min}-6\mu_{\max}-12 \alpha \sigma^{2}-\frac{2\sigma \Delta}{3\epsilon^{2/3} (\sigma(1+\alpha \Delta))^{1/3} }=0
\end{align*}
The solution of $\alpha$ that satisfies the equation above is negative, let us denote the solution by $-\alpha^{\star}$. 
Hence, finally we have that 
\begin{align*}
\norm{\mathcal{M}-\mathcal{M'}}_{TV} \ge \frac{1}{k} \exp\Big(\alpha^{\star}(6\mu_{\max}- \mu_{\min})-6(\alpha^{\star})^{2}\sigma^{2}-\Big(\frac{\sigma(1-\alpha^{\star} (\mu_{\max}-\mu_{\min}))}{\epsilon} \Big)^{2/3} \Big)
\end{align*}

==> proofpolyinterp.tex <==

Let $\bf{a}$ be the characteristic vector of a subset $S \subset \mathcal U$. Let $s_\ell=m_\ell(S)$ on this  set and let ${\bf s}=(s_0, s_1,\ldots, s_{k-1})$. We need to prove $\bf a$ is uniquely determined by $\bf s$.
%Then,
%\begin{align*}
%\sum_{j=1}^{n} a_j f(j)^i =m_k \quad \text{for } \mu=0,1,\dots,k-1
%\end{align*}
%and let $\mathcal{S}_k$ be the vector whose $jth$ component is $s_j$. Now, we study the necessary conditions on $\mathcal{B},k$ so that we can uniquely reconstruct $\mathbf{a}$.
%% Now, we can write $\mathcal{B}_j=p(j)$ where $p(j)$ is a polynomial of degree at most $d \le \sqrt{n}$.   
%Now, let us define a function $f:\mathbb{R}\rightarrow \mathbb{R}$ such that $\mathcal{B}(j)=f(j)$ for $j=0,\dots,n-1$.

Define
\begin{align*}
n_{i,p}(\mathbf{a})=\sum_{f(r)\equiv_p f(i)} a_{r} \pmod{p}
\end{align*}
Recall that Fermat's theorem (\cite{hardy1979introduction}) says that for any prime $p$ and any number $\alpha \not \equiv_p 0$, we must have that $\alpha^{p-1} \equiv_p 1$. Hence, for a prime number $p$ and some number $f(i) \not \equiv_p 0$, we have 
\begin{align*}
s_{0}(\mathbf{a)}-\sum_{j} {p-1 \choose j} s_j (-f(i))^{p-1-j} 
&\equiv_p \sum_{r} a_r -\sum_{j} {p-1 \choose j} \sum_{r} a_r f(r)^{j} (-f(i))^{p-1-j} \\
&\equiv_p  \sum_{r} a_r -\sum_{r} a_r  \sum_{j} {p-1 \choose j} f(r)^{j} (-f(i))^{p-1-j} \\
&\equiv_p  \sum_{r} a_r -\sum_r a_r (f(r)-f(i))^{p-1} \\
&\equiv_p \sum_{f(r) \equiv_p f(i)} a_r \equiv_p  n_{i,p} (\mathbf{a}) \ .
\end{align*}
%\andrew{reference Fermat's little theorem to explain second last line?}




Denote $\alpha_j$'s to be the coefficients of the degree $d$ polynomial $f$, i.e., $f(r)=\sum_{j=0}^{d} \alpha_j r^j$. 
Now, for a fixed $i$, $f(i)$ will be fixed and therefore the equation $f(r) \equiv_p f(i)$ can have at most $d$ distinct solutions in $r$.
 %\andrew{more detail here? why is this the form?}
 

These solutions look like $r \equiv_p \beta_j$  for $j=1,\dots,s$ where $s<d$. We have that 
\begin{align*}
n_{i,p}(\mathbf{a})=\sum_{f(r)\equiv_p f(i) } a_{r}=\sum_{j=1}^{s} \sum_{r \equiv_p \beta_j} a_r 
\end{align*}
Notice that the maximum value of $n_{i,p}$ is at most $\lceil dn/p \rceil$, therefore we can obtain the value of $n_{i,p}$ exactly if $p$ is chosen to be greater than $\sqrt{dn}$. Moreover, since the coefficients of the polynomial are rational the inverse of the denominator for every coefficient must exist. Since there are at most $d$ coefficients, at most $d$ primes are barred from being taken into consideration.  For a particular set $\mathcal{B}$, let $\mathcal{P}_{\mathcal{B}}$ be the set of allowed primes between $\sqrt{dn}$ and $k$. 

%For a particular value of $p$, $f(i)\equiv 0 \pmod{p}$ can have at most $d$ solutions and therefore the possible number of candidates for $i$ for a given prime $p$ is at least $p-d$. For a particular prime $p$ let $\mathcal{I}_p$ denote the set of allowed values for $i$. \\

 Now, let us denote the vector $\mathbf{v}_{i,p} \in \mathbb{F}_{2}^{n}$ where the $r$th entry is
\begin{align*}
v_{i,p}[r]=
\begin{cases} 1 & \text{ if } f(r) \equiv_p f(i)\\
0 &  \text{  otherwise }
\end{cases}
\end{align*} 
Consider two distinct characteristic vectors $\mathbf{a},\mathbf{b}$ corresponding to two different subsets $S,S' \subset \mathcal{U}$. Now, if $\bf{a}$ and $\bf{b}$ both give rise to the same vector $\bf{s}$, then $\mathbf{a}.\mathbf{v}_{i,p}=\mathbf{b}.\mathbf{v}_{i,p}$. Therefore, if the set of vectors 
\begin{align*}
\mathcal{S}=\{\mathbf{v}_{i,p} \mid p \in \mathcal{P}_{\mathcal{B}}, 0 \le i \le p-1  \}
\end{align*}
spans $\mathbb{F}_{2}^{n}$, then $\mathbf{a}.\mathbf{v}=\mathbf{b}.\mathbf{v}$ for any $v \in \mathbb{F}_2^n$ and we must have $\mathbf{a}=\mathbf{b}$ which will be a contradiction. Hence, in this case, two distinct characteristic vectors cannot lead to the same vector $\bf{s}$ and therefore on observing $\bf{s}$, we can obtain the characteristic vector which will be unique. Now, consider a subset $\mathcal{T} \subset \mathcal{S}$ defined by
\begin{align*}
\mathcal{T}=\{v_{i,p} \mid  p \in \mathcal{P}_{\mathcal{B}}, i \in \mathcal{I}_p \}
\end{align*}
where $\mathcal{I}_p \subseteq \{0,1,\dots,p-1\}$ is the largest set that satisfies the following conditions:
\begin{enumerate}
\item If $i \in \mathcal{I}_p$ then there does not exist $j \neq i$ and $j \in \mathcal{I}_p$ such that $f(j) \equiv_p f(i)$
\item There does not exist $i \in \mathcal{I}_p$ such that $f(i) \equiv_p f(0)$ 
\end{enumerate}
Clearly, $|\mathcal{I}_p| \ge \frac{p-d}{d}$ 
%where the extra $1$ is coming because one of $\gamma_j (\beta_j)^{-1}$ is zero and is already excluded.
Now, there are two possible cases. First, let us assume that the vectors in $\mathcal{T}$ are not all linearly independent. In that case, we must have a set of $m$ distinct tuples $(i_1,p_1),(i_2,p_2),\dots,(i_m,p_m)$ such that  
\begin{align*}
\sum_{j=1}^{m}  \mathbf{v}_{(i_j,p_j)}=0
\end{align*} 
Let us define another vector $\tilde{\mathbf{v}}$ (an infinite dimension extension of $\sum_{j=1}^{m}  \mathbf{v}_{(i_j,p_j)}$) where 
\begin{align*}
\tilde{\mathbf{v}}[\ell]=\sum_{j=1}^{m} \mathds{1}\Big[f(\ell) \equiv_{p_j} f(i_j)  \Big] 
\end{align*}
 Let us define the following system of equations for an integer $u$:  $u$ must satisfy $u \equiv_{p_1} i_1 $ and $r \equiv_{p_j} 0$ for all $j \ge 2$ and $p_j \neq p_1$. Such an $r$ exists by the Chinese remainder theorem and notice that for this value of $u$, we must have 
 \begin{align*}
 f(u) \equiv_{p_1} f(i_1) ~~\text{ and }~~ f(u) \not \equiv_{p_j} f(i_j) \mbox{ for all} ~ j \ge 2
\end{align*}  
This is because for $p_j \neq p_1$, $f(u) \not \equiv_{p_j} f(i_j)$ since $u \equiv_{p_j} 0$ and $f(i_j) \not \equiv_{p_j} f(0)$ due to our choice of $\mathcal{T}$. Again for $p_j=p_1$ where $j \neq 1$, $i_j$ is such that $f(i_j) \not \equiv_{p_1} f(i_1) $. Therefore, we must have $\tilde{\mathbf{v}}[u]=1$ and now, let $s$ be the smallest number such that $\tilde{\mathbf{v}}[s] \neq 0$. We must have that $s>n$ because of our assumption of linear dependence. Now consider the vector $\mathbf{v}_{t}=\sum_{j=1}^{m} \mathbf{v}^{\star}_{i_j,p_j,s-t}$ where 
\begin{align*}
v^{\star}_{i,p,c}[r]=
\begin{cases} 1 & \text{ if } f(r+c) \equiv_p f(i)\\
0 &  \text{  otherwise }
\end{cases}
\end{align*}
Now, $\mathbf{v}_{t}^{i}=0 \forall i<t $ and $\mathbf{v}_{t}^{t} \neq 0$. Now we claim that the vectors $\mathbf{v}_t$ is in the span of the set $\mathcal{S}$. To see this, assume that the equation $f(x)-f(y) \equiv_{p} 0$ can be written as the product of terms that look like $x-y-c$ or $x+y-c$ where $c$ is a constant i.e.
\begin{align*}
f(x)-f(y)  \equiv c_0 \prod_{j=1}^{d} (x \pm y -c_j)
\end{align*}  
where $c_0,\dots,c_j$ are constants. In that case, we must have that
\begin{align*}
\mathds{1} \Big[f(r+s-t) \equiv_{p_j} f(i_j) \Big]=\mathds{1} \Big[f(r) \equiv_{p_j} f(i_j-s+t) \Big] \quad \forall r
\end{align*}
Now $\mathbf{v}_{i_j-s+t,p_j}$ belongs to the set $\mathcal{S}$ and therefore our claim is proved.
Hence the set of vectors $\{ \mathbf{v}_t\}_{t=1}^{n}$ are in the span of the set $\mathcal{S}$ and also span $\mathbb{F}_{2}^{n}$. 

For the second case, assume that the vectors in $\mathcal{T}$ are independent. If $|\mathcal{T}|>n$, then our proof is complete as well. Now we must have that 
\begin{align*}
|\mathcal{T}| \ge \sum_{p \in \mathcal{P}_{\mathcal{B}}} \frac{p-d}{d}=(1+o(1))\sum_{p \in \mathcal{P}_{\mathcal{B}}} \frac{p}{d}
\end{align*}
From the Prime Number Theorem (see, e.g., \cite[Section 22.19.1]{hardy1979introduction}) we have for any $\eta>0$,
\begin{align*}
\pi (x+\eta x)-\pi (x)=\frac{\eta x}{\log x}+o\Big(\frac{x}{\log x}\Big)
\end{align*}
Therefore, $\sum_{p \le x} p \sim \frac{x^{2}}{2 \log x}$ where the sum is taken over all primes $p \le x$. Again, recall that $\mathcal{P}_{\mathcal{B}}$ contains all the primes in $[\sqrt{dn},k]$ barring at most $d$ of them. Hence, we have that 
\begin{align*}
|\mathcal{T}| > \frac{k^2}{2d \log k}-dk-\frac{dn}{\log n} >n
\end{align*}
and therefore $k$ has to be at least $d^{2}\sqrt{n \log n}$.

